PYROBOCOP: Python-based Robotic Control & Optimization Package for Manipulation

PYROBOCOP is a Python-based package for control, optimization and estimation of robotic systems described by nonlinear Differential Algebraic Equations (DAEs). In particular, the package can handle systems with contacts that are described by complementarity constraints and provides a general framework for specifying obstacle avoidance constraints. The package performs direct transcription of the DAEs into a set of nonlinear equations by performing orthogonal collocation on finite elements. PYROBOCOP provides automatic reformulation of the complementarity constraints that are tractable to NLP solvers to perform optimization of robotic systems. The package is interfaced with ADOL-C[1] for obtaining sparse derivatives by automatic differentiation and IPOPT[2] for performing optimization. We evaluate PYROBOCOP on several manipulation problems for control and estimation.

==> mechanics_formulation.tex <==
\section{Mechanics of Stable Placement}\label{sec:mechanics}
We make the following assumptions throughout the paper.
\begin{enumerate}
    \item The size of object is much bigger than the contact patch between the gripper and the object.
    \item The width of the object is much smaller than the length of the object, i.e., the stability margin of the object is negligible.
\end{enumerate}
The first assumption ensures that the object incurs rotational slip during the contact configuration considered in this paper. The second assumption is required to ensure that the object is always in the unstable configuration when a contact is established between the object and the environment. The second assumption is applicable for a wide variety of daily-use objects. We will see that this assumption is necessary to to resolve controller behavior during placement.
